Precise heavy-light meson masses and hyperfine splittings from lattice QCD including charm quarks in the sea

We present improved results for the B and D meson spectrum from lattice QCD including the effect of u/d,s and c quarks in the sea. For the B mesons the Highly Improved Staggered Quark action is used for the sea and light valence quarks and NonRelativistic QCD for the b quark including O(\alpha_s) radiative corrections to many of the Wilson coefficients for the first time. The D mesons use the Highly Improved Staggered Quark action for both valence quarks on the same sea. We find M_{B_s}-M_B=84(2) MeV, M_{B_s}=5.366(8) GeV, M_{B_c}=6.278(9) GeV, M_{D_s}=1.9697(33) GeV, and M_{D_s}-M_{D}=101(3) MeV. Our results for the B meson hyperfine splittings are M_{B^*}-M_{B}=50(3) MeV, M_{B_s^*}-M_{B_s}=52(3) MeV, in good agreement with existing experimental results. This demonstrates that our perturbative improvement of the NRQCD chromo-magnetic coupling works for both heavyonium and heavy-light mesons. We predict M_{B_c^*}-M_{B_c}=54(3) MeV. We also present first results for the radially excited B_c states as well as the orbitally excited scalar B_c0^* and axial vector B_c1 mesons.

==> tables/Bcmeson-results.tex <==
\begin{tabular}{llllllllllll}
Set & $am_{b}$ & $am_{c}$ & $am_s$ &
$aE_{\eta_c}$ & $aE_{D_s}$ &
$aE_{B_c}$  & $a\Delta^{\rm hyp}_{B_c}$ &   $a\Delta^{0^+-0^-}_{B_c}$ &  $a\Delta^{1^+-1^-}_{B_c}$
&$aE_{B_c'} - aE_{B_c}$ & $aE_{B_c^{*'}} - aE_{B_c^*}$
\\
\hline
1 & 3.297 & 0.826 & 0.0641 & 2.22508(7) & 1.48729(30) & 1.30409(14) & 0.03659(17) & 0.256(87) & 0.212(73) &  - &  - \\ 
2 & 3.263 & 0.818 & 0.0636 & 2.21032(4) & 1.47559(20) & 1.29702(10) & 0.03658(13) & 0.335(27) & 0.327(39) &  - &  - \\ 
3 & 2.66 & 0.645 & 0.0522 & 1.83967(5) & 1.21934(14) & 1.08866(5) & 0.03140(3) & 0.241(17) & 0.250(9) & 0.618(27) & 0.605(19)\\ 
4 & 2.62 & 0.627 & 0.0505 & 1.80351(3) & 1.19554(8) & 1.07252(4) & 0.03137(2) & 0.252(5) & 0.242(6) & 0.637(15) & 0.625(13)\\ 
5 & 1.91 & 0.434 & 0.0364 & 1.33307(4) & 0.88212(9) & 0.81480(3) & 0.02470(2) & 0.190(2) & 0.184(2) & 0.616(8) & 0.591(7)\\ 
\end{tabular}

==> tables/Bmeson-results.tex <==
\begin{tabular}{lllllllll}
Set & $am_b$ & $am_s$ & $am_l$ &  $aM_{\pi}$ & $aE(B_s)-aE(B)$ & $a\Delta^{\rm hyp}_{B}$ & $a\Delta^{0^+-0^-}_{B}$ &  $a\Delta^{1^+-1^-}_{B}$\\
\hline
1 & 3.297 & 0.0641 & 0.013 & 0.23637(15) & 0.05111(126) & 0.0375(12) & 0.245(17) & 0.251(20)\\ 
2 & 3.263 & 0.0636 & 0.0064 & 0.16615(7) & 0.05821(110) & 0.0377(9) & 0.207(25) & 0.150(57)\\ 
3 & 2.66 & 0.0522 & 0.01044 & 0.19153(9) & 0.04288(63) & 0.0324(4) & 0.193(13) & 0.192(15)\\ 
4 & 2.62 & 0.0505 & 0.00507 & 0.13413(5) & 0.04705(60) & 0.0309(4) & 0.200(4) & 0.207(4)\\ 
5 & 1.91 & 0.0364 & 0.0074 & 0.14070(9) & 0.03134(78) & 0.0212(11) & 0.159(8) & 0.158(7)\\ 
\end{tabular}

==> tables/Bmesonhyp-results.tex <==
\begin{tabular}{llllll}
Set& $a\Delta_{B}^{\mbox{\tiny hyp}}$ &$a\Delta_{B_s}^{\mbox{\tiny hyp}}$ & $a\Delta_{B_c}^{\mbox{\tiny hyp}}$ 
& $m_b^{\rm phys}$ & tuning \\
\hline
1 & 0.0375(12) & 0.03892(40) & 0.03659(17) & 3.297(11)(35)(7)(16) & 1.000(5)\\ 
2 & 0.0377(9) & 0.03705(47) & 0.03658(13) & 3.263(7)(35)(4)(16) & 1.000(5)\\ 
3 & 0.0324(4) & 0.03177(18) & 0.03140(3) & 2.696(4)(22)(7)(13) & 0.987(5)\\ 
4 & 0.0309(4) & 0.03102(16) & 0.03137(2) & 2.623(7)(22)(7)(13) & 0.999(6)\\ 
5 & 0.0212(11) & 0.02310(14) & 0.02470(2) & 1.893(6)(12)(5)(9) & 1.009(5)\\ 
\end{tabular}

==> tables/Bsmeson-results.tex <==
\begin{tabular}{lllllllllll}
  Set & $am_{b}$ & $aM_{b\overline{b}}$ 
  & $aE_{\eta_b}$ & $aE_{\Upsilon}$
  & $am_s$ & $aM_{\eta_s}$
   & $aE_{B_s}$  & $a\Delta^{hyp}_s$ & $a\Delta^{0^+-0^-}_{B_s}$ & $a\Delta^{1^+-1^-}_{B_s}$ \\ 
\hline
1 & 3.297 & 7.119(9) & 0.21289(6) & 0.26420(8) & 0.0641 & 0.51491(14) & 0.61558(47) & 0.03892(40) & 0.282(12) & 0.289(17)\\ 
2 & 3.263 & 7.040(8) & 0.21546(3) & 0.26669(5) & 0.0636 & 0.51078(8) & 0.61132(26) & 0.03705(47) & 0.285(5) & 0.280(8)\\ 
3 & 2.66 & 5.761(14) & 0.22040(5) & 0.26394(7) & 0.0522 & 0.42351(9) & 0.52385(23) & 0.03177(18) & 0.228(3) & 0.225(5)\\ 
4 & 2.62 & 5.719(7) & 0.22408(3) & 0.26767(5) & 0.0505 & 0.41476(6) & 0.52029(17) & 0.03102(16) & 0.218(6) & 0.222(4)\\ 
5 & 1.91 & 4.264(11) & 0.21519(2) & 0.24802(2) & 0.0364 & 0.30884(11) & 0.41051(17) & 0.02310(14) & 0.164(5) & 0.161(6)\\ 
\end{tabular}

==> tables/Dmeson-results.tex <==
\begin{tabular}{lllllllllll}
Set & $am_{c}$ & $am_{s}$ & $am_l$ &
$aE_{\eta_c}$ & $aE_{D_s}$ & $aE_{D}$ &
$aE_{D_s} - aE_{D}$  & $ aE_{D_s} - aE_{\eta_c}/2 $  
& $\Delta_{M_{\eta_s}^2 }$ &  $\Delta_{M_{\eta_c}}$
\\
\hline
1 & 0.826 & 0.0641 & 0.013 & 2.22508(7) & 1.48729(30) & 1.43326(58) & 0.05403(57) & 0.37475(29)&0.0&0.3\\ 
2 & 0.818 & 0.0636 & 0.0064 & 2.21032(4) & 1.47559(20) & 1.41258(68) & 0.06300(69) & 0.37043(19)&0.0&0.2\\ 
3 & 0.645 & 0.0522 & 0.01044 & 1.83967(5) & 1.21934(14) & 1.17112(53) & 0.04822(47) & 0.29950(13)&0.7&0.4\\ 
4 & 0.627 & 0.0505 & 0.00507 & 1.80351(3) & 1.19554(8) & 1.14112(61) & 0.05442(58) & 0.29379(8)&0.8&0.4\\ 
5 & 0.434 & 0.0364 & 0.0074 & 1.33307(4) & 0.88212(9) & 0.84682(26) & 0.03530(21) & 0.21559(10)&0.0&0.4\\ 
\end{tabular}

==> tables/bmeson-errorbudget.tex <==
\begin{table}[ht]
\begin{ruledtabular}
\begin{tabular}{lccc}
%\hline
%\hline
Error 				& $M_{B_s}$ & $M_{B_c, hh}$ & $M_{B_c, hs}$ \\
\hline
Stats/tuning/uncty in $a$  	& 4.8 	& 2.1 	& 9.5 	\\
Lattice spacing dependence 	& 2.2 	& 0.6 	& 3.5 	\\
$m_{b}$ dependence 		& 2.8 	& 2.9 	& 3.5  	\\
$m_{q,sea}$ dependence 		& 1.4 	& 1.4 	& 5.0  	\\
spin-ind. NRQCD systs. 		& 3.4 	& 5.3 	& 2.3	\\
spin-dep. NRQCD systs. 		& 3.0 	& 3.0 	& 0.0 	\\
uncty in $M_{\eta_s}$ 		& 0.3 	& - 	& 0.7	\\
em, annihiln in $b\overline{b}$ & 1.0   & $1.0^*$ & 0.0	\\
em, annihiln in $c\overline{c}$ & - 	& $1.5^*$ & 0.2 \\
em effects in $B_s$ or $B_c$ 	& 0.1 	& $1.0^*$ & 1.0 \\
em effects in $D_s$  		& - 	& - 	& 1.0 	\\
finite volume 			& 0.0 	& 0.0 	& 0.0 	\\
\hline
Total (MeV) 			& 7.7	& 8.0	& 12.2 \\
%\hline
%\hline
\end{tabular}
\end{ruledtabular}
\caption{\label{tab:errors} 
Full error budget 
for $B_s$ and $B_c$ meson masses in MeV. 
The source of each error is described in the text and the total error is
obtained by adding in quadrature.
Starred errors are correlated and are added linearly before 
being squared.
 }
\end{table}
